On the Trend-corrected Variant of Adaptive Stochastic Optimization Methods

Adam-type optimizers, as a class of adaptive moment estimation methods with the exponential moving average scheme, have been successfully used in many applications of deep learning. Such methods are appealing due to the capability on large-scale sparse datasets with high computational efficiency. In this paper, we present a new framework for Adam-type methods with the trend information when updating the parameters with the adaptive step size and gradients. The additional terms in the algorithm promise an efficient movement on the complex cost surface, and thus the loss would converge more rapidly. We show empirically the importance of adding the trend component, where our framework outperforms the conventional Adam and AMSGrad methods constantly on the classical models with several real-world datasets.

==> 3_convergence.tex <==
%%%%%%%%%%% Explanation: REGRET
\subsection{Backgrounds}
We investigate the convergence of AdamT with regret minimization by following \cite{zinkevich2003online}. Formally, the regret is defined as the difference between total cost and that of best point in hindsight 
$$
R(T)=\sum_{t=1}^{T}[f_{t}(x_{t})-f_{t}(x^{*})],
$$
where $f(x_t)$ is the convex function with arguments $x_t$ at iteration $t$ and $x^*$ denotes the optimal set of the parameters.%For the sake of clarity, we denote $f(x_t)$ as $f_t$.

For a vanishing average regret, Jensen's inequality implies that the average decision $f(\overline{x}_T)$ converges to $f(x^{*})$. In other words,
$$
f(\overline{x}_{T})-f(x^{*}) \leq \frac{1}{T} \sum_{t=1}^{T}\left[f(x_{t})-f(x^{*})\right]=\frac{\text { regret }}{T}.
$$
%In order to prove the converge of the algorithm, we instead prove $\frac{\text { regret }}{T} \rightarrow 0$ for $T \rightarrow \infty$.


%%%%%%%%%%% theorems
Below we list essential theorems and lemmas.

%\GaoC{Below are the definition for the convexity and subgradient, not Theorems!}
\begin{definition}[Convexity]
Let $\mathcal{K} \subseteq \mathbb{R}^{d}$ be a bounded convex and compact set in Euclidean space. A function $f: \mathcal{K} \mapsto \mathbb{R}$ is convex if for any $x, y \in \mathcal{K}$ 
$$
\forall \alpha \in[0,1],\qquad f(\alpha x+(1-\alpha) y) \leq \alpha f(x)+(1-\alpha) f(y).
$$
\label{convexity}
\end{definition}
We denote by $D$ an upper bound on the diameter of $\mathcal{K}$, then 
$$
x, y \in \mathcal{K},\quad \|x - y\| \leq D
$$

\begin{definition}[Subgradient]
The set of all subgradients of a function $f$ at $x$, denoted $\partial f(x)$, is the set of all vectors $u$ such that
$$
f(y) \geq f(x)+u^{\top}(y-x)
$$
\label{subgradient}
\end{definition}

%\begin{corollary}
Suppose $f$ is differentiable, for any existing gradient $\nabla f(x)$, we have $\nabla f(x) \in \partial f(x)$ and $\forall y \in \mathcal{K}$
$$
f(y) \geq f(x)+\nabla f(x)^{\top}(y-x).
$$
%\end{corollary}

We denote $G \geq 0$ and upper bound on the norm of the subgradients of $f$ over $\mathcal{K}$, i.e., $\|\nabla f(x)\| \leq G$ %\GaoC{$\|\partial f(\mathbf{x})\| \leq G$?} 
for all $x \in \mathcal{K}$. In other words, the function $f$ is Lipschitz continuous with parameter $G$, that is, for all $x, y \in \mathcal{K}$
$$
|f(x) - f(y)| \leq G\|x-y\|
$$

%%%%%%%%%%% lemmas
Below are the three core lemmas that applied in proving the regret bound.

\begin{lemma}[\cite{kingma2014adam}]
We define $\nabla f_{1:t,i} \in \mathbb{R}^t$ as the vector at the $i^{th}$ dimension of the gradients over all iterations till t, $\nabla f_{1:t,i} = [\nabla f_{1,i}, \nabla f_{2,i}, ..., \nabla f_{t,i}]$. With $\|\nabla f_{t}(x_t)\|_2 \leq G,\, \|\nabla f_{t}(x_t)\|_{\infty} \leq G_{\infty}$ we have
$$\sum_{t=1}^{T} \sqrt{\frac{\nabla f_{t, i}^{2}}{t}} \leq 2 G_{\infty}\left\|\nabla f_{1:T,i}\right\|_{2}
$$
\label{lemma3}
\end{lemma}

\begin{lemma}
For $\beta_1,\gamma_1,\beta_2,\gamma_2\in[0,1)$ and $\phi_1,\phi_2\in[0, 1]$ the series $\{\hat{m}_{t,i}\}$ and $\{\hat{v}_{t,i}\}$ has the following summation form
$$
\begin{aligned}
\hat{m}_{t,i} \leq \left[\frac{(1-\beta_1)}{1-\beta_{1}^{t}}+\frac{(1-\gamma_1 \phi_1)(1-\beta_{1})}{(1-(\gamma_{1}\phi_{1})^{t})} \right] \sum_{i=1}^{t} \nabla f_i.\\
\hat{v}_{t,i} \leq \left[\frac{(1-\beta_2)}{1-\beta_{2}^{t}}+\frac{(1-\gamma_2 \phi_2)(1-\beta_{2})}{(1-(\gamma_{2}\phi_{2})^{t})} \right] \sum_{i=1}^{t} \nabla f_i^2.
\end{aligned}
$$
\label{lemma4}
\end{lemma}

\begin{proof}
We start from $\hat{m}_{t,i}$. It can be shown that 
% error correction form
$$
\begin{aligned}
m_{t-1} &= \ell_{t-1}^{m} + \phi_1 b_{t-1}^{m} \\
\ell_{t}^{m} &= (1-\beta_{1}) \nabla f_t + \beta_1 l_{t-1}^m + \beta_1 \phi_1 b_{t-1}^m\\
b_{t}^{m} &= (1 - \beta_{1})(1 - \gamma_{1}) \nabla f_t - (1 - \beta_{1})(1 - \gamma_{1}) l_{t-1}^m - ((1 - \beta_{1})(1 - \gamma_{1})  - \phi_1) b_{t-1}^m\\
\end{aligned}
$$

Substitute $\ell_{t,i}^m$ and $b_{t,i}^m$, we have
% summation of m with g_i
$$
\begin{aligned}
\hat{m}_{t,i} =& \frac{1}{1-\beta_{1}^{t}}\ell_{t,i}^{m}+\frac{(1-\gamma_1 \phi_1)}{(1-\gamma_{1})(1-(\gamma_{1}\phi_{1})^{t})} b_{t,i}^{m}\\
=& \left[\frac{(1-\beta_1)}{1-\beta_{1}^{t}}+\frac{(1-\gamma_1 \phi_1)(1-\beta_{1})}{(1-(\gamma_{1}\phi_{1})^{t})} \right] \nabla f_{t,i}\\
&+ \left[\frac{(1-\beta_1)}{1-\beta_{1}^{t}} (\beta_1(1+\phi_1))
+\frac{(1-\gamma_1\phi_1)(1-\beta_{1})}{(1-(\gamma_{1}\phi_{1})^{t})} (\phi_1 - (1-\beta_1)(2-\gamma_1))
\right] \nabla f_{t-1,i}\\
&+ \left[\frac{(1-\beta_1)}{1-\beta_{1}^{t}} (\beta_1((\beta_1 - \phi_1(1-\beta_1)(1-\gamma_1))+\phi_1)(\beta_1 - \phi_1 + (1-\beta_1)(1-\gamma_1)))\right.\\
&\hspace{-.3cm}+\left.\frac{(1-\gamma_1\phi_1)(1-\beta_{1})}{(1-(\gamma_{1}\phi_{1})^{t})} 
(\beta_1(1-\beta_1)(\phi_1(\gamma_1-1) - 1) - (\phi_1 - (1-\beta_1)(2-\gamma_1))((1-\beta_1)(1-\gamma_1)-\phi_1))
)\right] \nabla f_{t-2,i} \\
&+ \cdots\\
&\leq \left[\frac{(1-\beta_1)}{1-\beta_{1}^{t}}+\frac{(1-\gamma_1 \phi_1)(1-\beta_{1})}{(1-(\gamma_{1}\phi_{1})^{t})} \right] \sum_{k=1}^{t} \nabla f_{k,i}
\end{aligned}
$$

Similarly for $\hat{v}_t$, we have
$$
\hat{v}_{t,i} \leq \left[\frac{(1-\beta_2)}{1-\beta_{2}^{t}}+\frac{(1-\gamma_2 \phi_2)(1-\beta_{2})}{(1-(\gamma_{2}\phi_{2})^{t})} \right] \sum_{k=1}^{t} \nabla f_{k,i}^2.
$$

\end{proof}


\subsection{Proof of regret bound}
%%%%%%%%%%% target
% assumption

% conclusion
\begin{theorem}
Assume that the objective function $f_t$ has bounded gradients, that is $\|\nabla f_t(x)\|_2\leq G$, $\|\nabla f_t(x)\|_{\infty}\leq G_{\infty}$ for all $x\in\R^d$. We further assume that the distance between any $x_t$ produced by AdamT is bounded, that is $\|x_n-x_m\|_2\leq D$, $\|x_m-x_n\|_{\infty}\leq D_{\infty}$ for any $m,n\in\{1,2,\ldots,T\}$, and $\beta_1,\gamma_1,\beta_2,\gamma_2\in[0,1)$, $\phi_1,\phi_2\in[0, 1]$. The proposed AdamT achieves the following guarantee for all $T\geq 1$
\begin{align*}
R(T)\leq& \frac{D^2_{\infty}}{2\eta(1-\beta_1)}\sum_{i=1}^d\sqrt{T\hat{v}_{T, i}} 
+ 
\frac12[\beta_1(1-\beta_1)(1 + \phi_1(1-\gamma_1))^2]G^2_{\infty}+\frac{2(1-\gamma_1\phi_1)^3}{(1-\beta_1)((1-\gamma_1)(1-(\gamma_1\phi_1)^T))^2}D^2_{\infty}\\
&+ 
\frac{\eta}{2(1-\beta_1)}
\frac{(2-\beta_1)^2}{\sqrt{2-\beta_2}} \sum_{i=1}^d \|g_{1:T,i}\|_2
+ 
d D^2_{2}\frac{(1-\gamma_1)\beta_1+1-\gamma_1\phi_1}{2(1-\gamma_1)(1-\beta_1)}
\end{align*}
\end{theorem}


%%%%%%%%%%% proof
\begin{proof}
According to Theorem \ref{subgradient}, for any convex function $f_t$ and $x^* \in \mathcal{K}$, we have
$$
f_{t}(x_{t})-f_{t}(x^{*}) \leq \nabla f_t(x_t)^{\top}(x_t-x^*)
$$
which implies the regret upper bound
$$
R(T) = \sum_{t=1}^{T}f_{t}(x_{t})-\sum_{t=1}^{T}f_{t}(x^{*}) 
\leq \sum_{t=1}^{T}\nabla f_t(x_t-x^*).
$$

From the update rules in Algorithm, %\ref{algo1}
$$
\begin{aligned}
x_{t+1} &= x_{t} - \frac{\eta_t}{\sqrt{\hat{v}_{t}}}\,\hat{m}_{t}\\
%{\lvert\hat{v}_{t}\rvert^{1/2}}\,\hat{m}_{t}
&= x_{t} - \frac{\eta_t}{\sqrt{\hat{v}_{t}}}\left(\frac{\ell_{t}^{m}}{1-\beta_{1}^{t}}+\frac{(1-\gamma_1\phi_1) b_{t}^{m}}{(1-\gamma_{1})(1-(\gamma_{1}\phi_1)^{t})}\right)\\
&= x_{t} - \frac{\eta_t}{\sqrt{\hat{v}_{t}}}\left(\frac{\beta_{1}(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})}{1-\beta_{1}^{t}}+\frac{(1-\beta_{1}) \nabla f_t(x_t)}{1-\beta_{1}^{t}}+\frac{(1-\gamma_1\phi_1) b_{t}^{m}}{(1-\gamma_{1})(1-(\gamma_{1}\phi_1)^{t})}\right).
\end{aligned}
$$

Consider the $i^{th}$ dimension of the parameter vector at time $t$
$$
\begin{aligned}
(x_{t+1,i} - x^*_{i})^2 =& (x_{t,i} - \frac{\eta_t}{\sqrt{\hat{v}_{t,i}}}\,\hat{m}_{t,i} - x^*_{i})^2 \\
=& (x_{t,i} - x^*_{i})^2 - 2\eta_t \frac{\hat{m}_{t,i}}{\sqrt{\hat{v}_{t,i}}}(x_{t,i} - x^*_{i}) + \eta_t^2 (\frac{\hat{m}_{t,i}}{\sqrt{\hat{v}_{t,i}}})^2\\
=& (x_{t,i} - x^*_{i})^2 - 
\frac{2\eta_t}{\sqrt{\hat{v}_{t}}}\left(\frac{\beta_{1}(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})}{1-\beta_{1}^{t}}+\frac{(1-\beta_{1}) \nabla f_t(x_t)}{1-\beta_{1}^{t}}+\frac{(1-\gamma_1\phi_1) b_{t}^{m}}{(1-\gamma_{1})(1-(\gamma_{1}\phi_1)^{t})}\right)
(x_{t,i} - x^*_{i}) \\
&+ \eta_t^2 (\frac{\hat{m}_{t,i}}{\sqrt{\hat{v}_{t,i}}})^2\\
\end{aligned}
$$

Rearrange the equation above will get
$$
\begin{aligned}
\nabla f_{t,i}(x_{t,i} - x^*_{i})
=& \frac{\sqrt{\hat{v}_{t}}(1-\beta_{1}^{t})}{2\eta_t(1-\beta_{1})}\left((x_{t,i} - x^*_{i})^2 - (x_{t+1,i} - x^*_{i})^2\right) \\
&- \left(\frac{\beta_{1}(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})}{1-\beta_{1}}+\frac{(1-\beta_{1}^{t})(1-\gamma_1\phi_1)b_{t}^{m}}{(1-\beta_{1})(1-\gamma_1)(1-(\gamma_{1}\phi_1)^{t})}\right)(x_{t,i} - x^*_{i}) + 
\frac{\eta_t(1-\beta_{1}^{t})\hat{m}_{t,i}^2}{2(1-\beta_{1})\sqrt{\hat{v}_{t,i}}} \\
=& \frac{\sqrt{\hat{v}_{t}}(1-\beta_{1}^{t})}{2\eta_t(1-\beta_{1})}\left((x_{t,i} - x^*_{i})^2 - (x_{t+1,i} -x ^*_{i})^2\right) + \frac{\beta_{1}(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})}{1-\beta_{1}}(x^*_{i} - x_{t,i}) \\ 
&+ \frac{(1-\beta_{1}^{t})(1-\gamma_1\phi_1)b_{t}^{m}}{(1-\beta_{1})(1-\gamma_1)(1-(\gamma_{1}\phi_1)^{t})}
(x^*_{i} - x_{t,i}) + 
\frac{\eta_t(1-\beta_{1}^{t})\hat{m}_{t,i}^2}{2(1-\beta_{1})\sqrt{\hat{v}_{t,i}}}.
\end{aligned}
$$

For any $\beta_1 \leq 1$ and $(1-\beta_1^t) \leq 1$, we can get
$$
\begin{aligned}
\nabla f_{t,i}(x_{t,i} - x^*_{i}) \leq &
\frac{\sqrt{\hat{v}_{t}}}{2\eta_t(1-\beta_{1})}\left((x_{t,i} - x^*_{i})^2 - (x_{t+1,i} - x^*_{i})^2\right) + \frac{\beta_{1}(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})}{1-\beta_{1}}(x^*_{i} - x_{t,i}) \\ 
&+ \frac{(1-\gamma_1\phi_1)b_{t}^{m}}{(1-\beta_{1})(1-\gamma_1)(1-(\gamma_{1}\phi_1)^{t})}
(x^*_{i} - x_{t,i}) + 
\frac{\eta_t\hat{m}_{t,i}^2}{2(1-\beta_{1})\sqrt{\hat{v}_{t,i}}}.
\end{aligned}
$$

Applying Young's inequality on the second and the third term yields
$$
\begin{aligned}
&\frac{\beta_{1}(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})}{1-\beta_{1}}(x^*_{i} - x_{t,i})\\
=& \left(\sqrt{\frac{\beta_{1}}{(1-\beta_{1})}}
%\frac{1}{\sqrt{\eta_t}} 
(x^*_{i} - x_{t,i})\right)\left(\sqrt{\frac{\beta_{1}}{(1-\beta_{1})}}%\sqrt{\eta_t}
(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})
\right)\\ 
\leq& \frac{\beta_{1}}{2(1-\beta_{1})}%\frac{1}{\sqrt{\eta_t}}
(x^*_{i} - x_{t,i})^2
+ \frac{\beta_{1}}{2(1-\beta_{1})}%\sqrt{\eta_t}
(\ell_{t-1}^{m} + \phi_1 b_{t-1}^{m})^2, \\
&\frac{(1-\gamma_1\phi_1)b_{t}^{m}}{(1-\beta_{1})(1-\gamma_1)(1-(\gamma_{1}\phi_1)^{t})}
(x^*_{i} - x_{t,i}) \\
=& \left(\sqrt{\frac{1-\gamma_1\phi_{1}}{(1-\beta_{1})(1-\gamma_1)}}%\frac{1}{\sqrt{\eta_t}}
(x^*_{i} - x_{t,i})\right)\left(\sqrt{\frac{\phi_{1}}{(1-\beta_{1})}}%\sqrt{\eta_t}
\frac{b_t^m}{(1 - \gamma_1^t)}
\right)\\ 
\leq& \frac{1-\gamma_1\phi_{1}}{2(1-\beta_{1})(1-\gamma_1)} %\frac{1}{\eta_t}
(x^*_{i}-x_{t,i})^2
+ \frac{1-\gamma_1\phi_{1}}{2(1-\beta_{1})(1-\gamma_1)}%\eta_t
\left(\frac{b_t^{m}}{(1 - \gamma_1^t)}\right)^2 \\
\end{aligned}
$$

The regret bound can be derived by taking summation across all the dimensions for $i = 1, 2,\ldots, d$ and the convex functions for $t = 1, 2, \ldots, T$. 

\begin{align*}
R(T) &\leq \sum_{i=1}^{d}\sum_{t=1}^{T}\nabla f_{t,i}(x_{t,i}-x_{i}^*)\\
&\leq \underbrace{\sum_{i=1}^d \frac{1}{2\eta(1-\beta_1)}(x_{1,i}-x_{i}^*)^2\sqrt{\hat{v}_{1, i}}+\sum_{i=1}^d\sum_{t=2}^T\frac{1}{2(1-\beta_1)}(x_{t,i}-x_{i}^*)^2\left(\frac{\sqrt{\hat{v}_{t,i}}}{\eta}-\frac{\sqrt{\hat{v}_{t-1, i}}}{\eta_{t-1}}\right)}_{P1}\\
&+\underbrace{\sum_{t=1}^T\frac{1}{2(1-\beta_1)}\left(\beta_1(\ell_{t-1}^m+\phi_1 b_{t-1}^m)^2+\frac{(1-\gamma_1\phi_1)((1-\gamma_1\phi_1)(b_t^m))^2}{((1-\gamma_1)(1-(\gamma_1\phi_1)^T))^2}\right)}_{P2}\\
&+\underbrace{\sum_{i=1}^d\sum_{t=1}^T\frac{\eta}{2(1-\beta_1)}\frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}}}}_{P3}
+\underbrace{\sum_{t=1}^T\frac{1}{2(1-\beta_1)}\left(\beta_1 + \frac{1-\gamma_1\phi_1}{1-\gamma_1}\right)(x_{i}^*-x_{t, i})^2}_{P4}
\end{align*}

According to the assumptions $\|x_{t}-x^{*}\|_{2} \leq D$, $\|x_{m}-x_{n}\|_{\infty} \leq D_{\infty}$ for any $m,n \in {1, 2,\ldots, T}$, the above four parts in the inequality can be further upper bounded as follows respectively:
\begin{align*}
P1 &= \sum_{i=1}^d \frac{1}{2\eta(1-\beta_1)}(x_{1,i}-x_{i}^*)^2\sqrt{\hat{v}_{1, i}}+\sum_{i=1}^d\sum_{t=2}^T\frac{1}{2(1-\beta_1)}(x_{t,i}-x_{i}^*)^2\left(\frac{\sqrt{\hat{v}_{t,i}}}{\eta_t}-\frac{\sqrt{\hat{v}_{t-1, i}}}{}\right)\\
&\leq\frac{D^2_{\infty}}{2\eta(1-\beta_1)}\sum_{i=1}^d\sqrt{T\hat{v}_{T, i}}\\
%%%
P2 &= \sum_{t=1}^T\frac{1}{2(1-\beta_1)}\left(\beta_1(\ell_{t-1}^m+\phi_1 b_{t-1}^m)^2+\frac{(1-\gamma_1\phi_1)((1-\gamma_1\phi_1)(b_t^m))^2}{((1-\gamma_1)(1-(\gamma_1\phi_1)^T))^2}\right)\\
&= \sum_{t=1}^T\frac{\beta_1}{2(1-\beta_1)}(\ell_{t-1}^m+\phi_1 b_{t-1}^m)^2 + \sum_{t=1}^T\frac{1}{2(1-\beta_1)}\frac{(1-\gamma_1\phi_1)((1-\gamma_1\phi_1)(b_t^m))^2}{((1-\gamma_1)(1-(\gamma_1\phi_1)^T))^2}\\
&\leq \frac12(\beta_1(1-\beta_1)(1 + \phi_1(1-\gamma_1))^2)
\sum_{t=1}^T\nabla f_{t-1}^2\\
&+ \frac{(1-\gamma_1\phi_1)^3}{2(1-\beta_1)((1-\gamma_1)(1-(\gamma_1\phi_1)^T))^2} \sum_{t=1}^T (b_t^m)^2\\
&\leq \frac12(\beta_1(1-\beta_1)(1 + \phi_1(1-\gamma_1))^2)G^2_{\infty}+\frac{2(1-\gamma_1\phi_1)^3}{(1-\beta_1)((1-\gamma_1)(1-(\gamma_1\phi_1)^T))^2}D^2_{\infty}\\
%%%
P3 &= \sum_{i=1}^d\sum_{t=1}^T\frac{\eta}{2(1-\beta_1)}\frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}}} \leq \frac{\eta}{2(1-\beta_1)}
\frac{(2-\beta_1)^2}{\sqrt{2-\beta_2}} \sum_{i=1}^d \|g_{1:T,i}\|_2\\
%%%
P4 &= \sum_{i=1}^d\sum_{t=1}^T\frac{1}{2(1-\beta_1)}\left(\beta_{1} + \frac{1-\gamma_1\phi_1}{1-\gamma_1}\right)(x_{i}^*-x_{t, i})^2\\
&\leq \frac{(1-\gamma_1)\beta_1+1-\gamma_1\phi_1}{2(1-\gamma_1)(1-\beta_1)}\sum_{i=1}^d D^2_{2}\\
&=d D^2_{2}\frac{(1-\gamma_1)\beta_1+1-\gamma_1\phi_1}{2(1-\gamma_1)(1-\beta_1)}
\end{align*}

Hence, the final regret upper bound can be written as:
\begin{align*}
R(T)\leq& \frac{D^2_{\infty}}{2\eta(1-\beta_1)}\sum_{i=1}^d\sqrt{T\hat{v}_{T, i}} 
+ 
\frac12[\beta_1(1-\beta_1)(1 + \phi_1(1-\gamma_1))^2]G^2_{\infty}+\frac{2(1-\gamma_1\phi_1)^3}{(1-\beta_1)((1-\gamma_1)(1-(\gamma_1\phi_1)^T))^2}D^2_{\infty}\\
&+ 
\frac{\eta}{2(1-\beta_1)}
\frac{(2-\beta_1)^2}{\sqrt{2-\beta_2}} \sum_{i=1}^d \|g_{1:T,i}\|_2
+ 
d D^2_{2}\frac{(1-\gamma_1)\beta_1+1-\gamma_1\phi_1}{2(1-\gamma_1)(1-\beta_1)}
\end{align*}

\end{proof}



